A 10.24-GHz-wide digital spectrometer array system for LMT-FINER: system design and laboratory performance verification

For efficient spectroscopic redshift identification of early galaxies in the northern hemisphere, we aim to combine the Large Millimeter Telescope (LMT) with a wide-band heterodyne receiver, FINER, which will cover radio frequencies of 120--360 GHz and offer a 3--21 GHz intermediate frequency (IF) per sideband and polarization. To take full advantage of such wide IFs, we present a novel 10.24-GHz-wide digital spectrometer, DRS4 (Elecs Industry Co., Ltd.). It incorporates 20.48 Gsps samplers with an FPGA-based digital signal processing module. To mitigate the noise contamination from the image sideband, it is equipped with a digital sideband separation function to improve the sideband rejection up to 25 dB. Laboratory performance evaluations show that it exhibits an Allan time of at least ~100 s and a total power dynamic range of at least 7 dB. These results demonstrate its capability of instantaneously wide-band spectroscopy toward high-redshift galaxies with position-switching observations.

==> Contents/Labexp_DSBS.tex <==
\subsection{Digital side-band separation}
\label{sec:lab_DSBS}
